Continual 3D Convolutional Neural Networks for Real-time Processing of Videos

We introduce Continual 3D Convolutional Neural Networks (Co3D CNNs), a new computational formulation of spatio-temporal 3D CNNs, in which videos are processed frame-by-frame rather than by clip. In online tasks demanding frame-wise predictions, Co3D CNNs dispense with the computational redundancies of regular 3D CNNs, namely the repeated convolutions over frames, which appear in overlapping clips. We show that Continual 3D CNNs can reuse preexisting 3D-CNN weights to reduce the per-prediction floating point operations (FLOPs) in proportion to the temporal receptive field while retaining similar memory requirements and accuracy. This is validated with multiple models on Kinetics-400 and Charades with remarkable results: CoX3D models attain state-of-the-art complexity/accuracy trade-offs on Kinetics-400 with 12.1-15.3x reductions of FLOPs and 2.3-3.8% improvements in accuracy compared to regular X3D models while reducing peak memory consumption by up to 48%. Moreover, we investigate the transient response of Co3D CNNs at start-up and perform extensive benchmarks of on-hardware processing characteristics for publicly available 3D CNNs.

==> bios.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author-lukas-new.jpeg}}]{Lukas Hedegaard Morsing}
is a PhD student at Aarhus University, Denmark. He received his M.Sc. degree in Computer Engineering in 2019 and B.Eng. degree in Electronics in 2017 at Aarhus University, specialising in signal processing and machine learning. His current research interests include deep learning and transfer learning focused on efficient utilisation of training data and computational resources.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author-alexandros}}]{Alexandros Iosifidis} (SM'16) is an Associate Professor of Machine Learning at the Department of Engineering, Aarhus University, Denmark. He received the B.Sc. degree in Electrical and Computer Engineering and the M.Sc. degree with a specialisation in Mechatronics from the Democritus University of Thrace, Greece, in 2008 and 2010, respectively. He also received his PhD in Computer Science from the Aristotle University of Thessaloniki, Greece, in 2014. Before he joined Aarhus University, he held Postdoctoral Researcher positions at Aristotle University of Thessaloniki and at Tampere University of Technology, Finland, where he was an Academy of Finland Postdoctoral Research Fellow. 

Dr. Iosifidis has contributed in more than twenty R\&D projects financed by EU, Finnish and Danish funding agencies and companies. He has (co-)authored 73 articles in international journals and 89 papers in international conferences proposing novel Machine Learning techniques and their application in a variety of problems. He is a Senior Member of IEEE since 2016, and he served as an Officer of the Finnish IEEE Signal Processing-Circuits and Systems Chapter during 2016-2018. He is currently a member of the EURASIP Technical Area Committee on Visual Information Processing, and serves as Area/Associate Editor in Neurocomputing, Signal Processing: Image Communications, IEEE Access and BMC Bioinformatics journals. He served as an Area Chair for IEEE ICIP-2018,2019,2020 and EUSIPCO-2019, Technical Program Committee Chair for IEEE ICASSP-2019, and he is the Publicity co-Chair of IEEE ICME-2021. His research interests focus on topics of neural networks and statistical machine learning finding applications in computer vision, financial engineering and graph mining problems.
\end{IEEEbiography}

==> content/05-oad-experiment.tex <==

\subsection{Online Action Detection} \label{sec:exp-oad}
Many existing Online Action Detection (OAD) methods, e.g. \cite{gao2017red}, \cite{xu2019temporal}, \cite{Eun2020LearningTD}, \cite{wang2021oadtr}, employ a standard pipeline to extract image and motion features by means of computationally expensive deep neural networks, on top of which the proposed OAD method is applied.
The image features are commonly extracted with ResNet-200~\cite{he2016resnet} (15.0 GFLOPs/frame, 64.7 M parameters~\cite{wang2017residual}) and optical flow is calculated using FlowNet V2~\cite{ilg2017flownet2} (44.9 GFLOPs/frame, 162.5 M parameters at input resolution $224 \times 224$) with subsequent feature-extraction using BN-Inception~\cite{ioffe2015batch} (2.0 GFLOPs/frame, 6.3 M parameters ~\cite{bianco2018benchmark}).
The resulting complexity of pre-processing totals an astounding 61.9 GFLOPs/frame and 233.5 M parameters, not counting the OAD method itself!
Such a heavy computational cost and memory footprint is ill-suited for real-life online inference systems; despite their performance gap, we would argue that lightweight methods such as Continual 3D CNNs are more applicable in real-life online scenarios.
For instance, \textit{Co}X3D-S lowers the computational complexity by $295\times$ and memory by $45\times$ compared to the above-described pre-processing pipeline.

Following the evaluation protocols of existing OAD methods~\cite{gao2017red}, \cite{xu2019temporal}, \cite{kim2021temporally}, \cite{Eun2020LearningTD}, \cite{wu2019long}, \cite{xu2021long}, \cite{wang2021oadtr}, \cite{Zhao2020PrivilegedKD}, we report the frame-level mean Average Precision (mAP) on THUMOS-14~\cite{idrees2017thumos} and the mean calibrated Average Precision (mcAP) on TVSeries~\cite{geest2016online} in ~\cref{tab:oad}. Here, the \textit{Co}X3D networks were initialised with X3D weights trained on Kinetics and finetuned on the target dataset without any network modifications.


\begin{table}
	\begin{center}
    % \resizebox{\linewidth}{!}{
	\begin{tabular}{lccc}
		\toprule
		\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{FLOPs} (G)}  & \textbf{Pre-}      & \multirow{2}{*}{\textbf{mcAP} (\%)}  \\
		                                 &              &\textbf{training}   & \\
		\midrule
% 		RED~\cite{gao2017red}           & $61.9+$ & \multirow{7}{*}{A.Net}        & $79.2$ \\
% 		TRN~\cite{xu2019temporal}       & $61.9+$ &                               & $83.7$ \\
% 		FATS~\cite{kim2021temporally}   & &                                       & $81.7$\\
% 		IDN~\cite{Eun2020LearningTD}    & $61.9+$ &                               & $84.7$ \\
% 		LFB~\cite{wu2019long,xu2021long}& &                                       & $84.8$\\
% 		OadTR~\cite{wang2021oadtr}      & $61.9+$ &                               & $85.4$ \\
% 		LSTR~\cite{xu2021long}          & &                                       & $88.1$ \\
% 		\midrule
		FATS~\cite{kim2021temporally}   & & \multirow{6}{*}{Kin.}                 & $84.6$\\
		IDN~\cite{Eun2020LearningTD}    & $61.9+$ &                               & $86.1$ \\
		LFB~\cite{wu2019long,xu2021long}& &                                       & $85.8$ \\
		PKD~\cite{Zhao2020PrivilegedKD} & &                                       & $86.4$ \\
		OadTR~\cite{wang2021oadtr}      & $61.9+$ &                               & $87.2$ \\
		LSTR~\cite{xu2021long}          & &                                       & $89.1$ \\
		\noalign{\vskip 2pt} \hdashline \noalign{\vskip 2pt}  
        \textit{Co}OadTr-X3D-L          & $1.5$ & \multirow{3}{*}{Kin.}           & - \\
        \textit{Co}OadTr-X3D-M          & $0.4$ &                                 & - \\
        \textit{Co}OadTr-X3D-S          & $0.2$ &                                 & - \\
		\bottomrule
	\end{tabular}
% 	}
% 	\vspace{-6pt}
	\caption{
	    \textbf{Online Action Detection}.
	    GFLOPs per frame: 
	    a) ResNet-200 (15.0), FlowNet V2 (44.9), BN-Inception (2.0)
	    b) ResNet-50 (3.8), DenseFlow (??), BN-Inception (2.0) % LSTR
	    \hl{TODO: check these}
	}
% 	\ificcvfinal \setlength{\belowcaptionskip}{-25pt} \fi
% 	\vspace{-15pt}
	\label{tab:oad}
	\end{center}
	\vspace{-8mm}
\end{table}

% \begin{table}
% 	\begin{center}
%     % \resizebox{\linewidth}{!}{
% 	\begin{tabular}{lcccccc}
% 		\toprule
% 		\multirow{2}{*}{\textbf{Model}} & \textbf{FLOPs}  & \textbf{Pre-}      & \textbf{THUMOS-14} & & \textbf{TVSeries} \\
% 		                                                                                            \cline{4-4}            \cline{6-6}
% 		                                 &\textbf{per frame (G)}               &\textbf{training}   & mAP (\%)           & & mcAP (\%) \\
% 		\midrule
% 		RED~\cite{gao2017red}           & $61.9+$ & \multirow{7}{*}{A.Net}        & $45.3$             & & $79.2$ \\
% 		TRN~\cite{xu2019temporal}       & $61.9+$ &                               & $47.2$             & & $83.7$ \\
% 		FATS~\cite{kim2021temporally}   & &                                       & $51.6$             & & $81.7$\\
% 		IDN~\cite{Eun2020LearningTD}    & $61.9+$ &                               & $50.0$             & & $84.7$ \\
% 		LFB~\cite{wu2019long,xu2021long}& &                                       & $61.6$             & & $84.8$\\
% 		OadTR~\cite{wang2021oadtr}      & $61.9+$ &                               & $58.3$             & & $85.4$ \\
% 		LSTR~\cite{xu2021long}          & &                                       & $65.3$             & & $88.1$ \\
% 		\midrule
% 		FATS~\cite{kim2021temporally}   & & \multirow{6}{*}{Kin.}                 & $59.0$             & & $84.6$\\
% 		IDN~\cite{Eun2020LearningTD}    & $61.9+$ &                               & $60.3$             & & $86.1$ \\
% 		LFB~\cite{wu2019long,xu2021long}& &                                       & $64.8$             & & $85.8$ \\
% 		PKD~\cite{Zhao2020PrivilegedKD} & &                                       & $64.5$             & & $86.4$ \\
% 		OadTR~\cite{wang2021oadtr}      & $61.9+$ &                               & $65.2$             & & $87.2$ \\
% 		LSTR~\cite{xu2021long}          & &                                       & $69.5$             & & $89.1$ \\
% 		\noalign{\vskip 2pt} \hdashline \noalign{\vskip 2pt}  
%         \textit{Co}OadTr-X3D-L          & $1.5$ & \multirow{3}{*}{Kin.}          & -                  & & - \\
%         \textit{Co}OadTr-X3D-M          & $0.4$ &                                & -                  & & - \\
%         \textit{Co}OadTr-X3D-S          & $0.2$ &                                & $29.4$             & & - \\
% 		\bottomrule
% 	\end{tabular}
% % 	}
% % 	\vspace{-6pt}
% 	\caption{
% 	    \textbf{Online Action Detection}.
% 	    GFLOPs per frame: 
% 	    a) ResNet-200 (15.0), FlowNet V2 (44.9), BN-Inception (2.0)
% 	    b) ResNet-50 (3.8), DenseFlow (??), BN-Inception (2.0) % LSTR
% 	    \hl{TODO: check these}
% 	}
% % 	\ificcvfinal \setlength{\belowcaptionskip}{-25pt} \fi
% % 	\vspace{-15pt}
% 	\label{tab:oad}
% 	\end{center}
% 	\vspace{-8mm}
% \end{table}

